A Minimal Framework for Optimizing Vaccination Protocols Targeting Highly Mutable Pathogens

A persistent public health challenge is finding immunization schemes that are effective in combating highly mutable pathogens such as HIV and influenza viruses. To address this, we analyze a simplified model of affinity maturation, the Darwinian evolutionary process B cells undergo during immunization. The vaccination protocol dictates selection forces that steer affinity maturation to generate antibodies. We focus on determining the optimal selection forces exerted by a generic time-dependent vaccination protocol to maximize production of broadly neutralizing antibodies (bnAbs) that can protect against a broad spectrum of pathogen strains. The model lends itself to a path integral representation and operator approximations within a mean-field limit, providing guiding principles for optimizing time-dependent vaccine-induced selection forces to enhance bnAb generation. We compare our analytical mean-field results with the outcomes of stochastic simulations and discuss their similarities and differences.

==> plots/V_n0.tex <==

\begin{axis}[
  axis x line=center,
  axis y line=none,
  xtick={0, 0.75, 1.1},
  xticklabels={0, $x_V$, $\ell$},
  ytick={-5,-4,...,5},
  tick style = {color=black},
  tick label style={font=\small},
  xlabel={$x$},
  ylabel={$y$},
  xlabel style={below right},
  ylabel style={above left},
  xmin=-.2,
  xmax=2.2,
  ymin=0,
  ymax=2.1,
  restrict y to domain=0:2.1,
  %enlarge x limits={rel=0.1},
  enlarge y limits={rel=1},
 ]
%Below the red parabola is defined
\addplot [
    domain=0.4:1.9, 
    samples=200, 
    color=blue,
    thick,
]
{exp(-20*(x-1.1)^2)} node[above,pos=0.5] {$n_0$};
%\addlegendentry{\(x^2 - 2x - 1\)}
%Here the blue parabola is defined
\draw [dotted, color=blue] (axis cs:1.1,0) -- (axis cs:1.1,1);
\addplot [
    domain=0.2:1.25, 
    samples=300, 
    color=red,
    thick,
    ]
    {2*exp(-20*(x-.75)^2)}
    node[above,pos=0.5] {$V$};;
%\addlegendentry{\(x^2 + 2x + 1\)}
\draw [dotted, color=red] (axis cs:.75,0) -- (axis cs:.75,2);
\end{axis}


==> plots/Vtilde_n0.tex <==
\begin{axis}[
  axis x line=center,
  axis y line=none,
  xtick={0.5, 1.1},
  xticklabels={$x_V\!-\!x^*$, $0$},
  ytick={-5,-4,...,5},
  tick style = {color=black},
  tick label style={font=\small},
  xlabel={$x$},
  ylabel={$y$},
  xlabel style={below right},
  ylabel style={above left},
  xmin=-.2,
  xmax=2.2,
  ymin=0,
  ymax=2.1,
  restrict y to domain=0:2.1,
  %enlarge x limits={rel=0.1},
  enlarge y limits={rel=1},
 ]
%Below the red parabola is defined
\addplot [
    domain=0.5:1.8, 
    samples=200, 
    color=blue,
    thick,
]
{exp(-20*(x-1.1)^2)} node[above,pos=0.5] {$n_0$};
%\addlegendentry{\(x^2 - 2x - 1\)}
%Here the blue parabola is defined
\draw [dotted, color=blue] (axis cs:1.1,0) -- (axis cs:1.1,1);
\addplot [
    domain=0:1, 
    samples=300, 
    color=red,
    thick,
    ]
    {2*exp(-20*(x-.5)^2)}
    node[above,pos=0.5] {$\widetilde{V}$};
%\addlegendentry{\(x^2 + 2x + 1\)}
\draw [dotted, color=red] (axis cs:.5,0) -- (axis cs:.5,2);
\end{axis}

==> plots/Vtilde_optimal.tex <==
\begin{axis}[
  axis x line=center,
  axis y line=none,
  xtick={0.5},
  xticklabels={$0$},
  ytick={-5,-4,...,5},
  tick style = {color=black},
  tick label style={font=\small},
  xlabel={$x$},
  ylabel={$y$},
  xlabel style={below right},
  ylabel style={above left},
  xmin=-.7,
  xmax=1.7,
  ymin=0,
  ymax=2.1,
  restrict y to domain=0:2.1,
  %enlarge x limits={rel=0.1},
  enlarge y limits={rel=1},
 ]
%Below the red parabola is defined
\addplot [
    domain=0:1.3, 
    samples=200, 
    color=blue,
    thick,
]
{exp(-20*(x-.5)^2)}; 
%node[above,pos=0.5] {$n_0$};

%\draw [dotted, color=blue] (axis cs:1.1,0) -- (axis cs:1.1,1);
\addplot [
    domain=0:1, 
    samples=300, 
    color=red,
    thick,
    ]
    {2*exp(-20*(x-.5)^2)}
    node[above,pos=0.5] {$\widetilde{V}$};
%\addlegendentry{\(x^2 + 2x + 1\)}
\draw [dotted, color=red] (axis cs:.5,0) -- (axis cs:.5,2);
\end{axis}
